Theoretical Study of Reactivity Indices and Rough Potential Energy Curves for the Dissociation of 59 Fullerendiols in Gas-Phase and in Aqueous Solution with an Implicit Solvent Model

Buckminsterfullerene, C$_{60}$, has not only a beautiful truncated icosahedral (soccerball) shape, but simple H\"uckel calculations predict a three-fold degenerate lowest unoccupied molecular orbital (LUMO) which can accomodate up to six electrons making it a good electron acceptor. Experiments have confirmed that C60 is a radical sponge and it is now sold for use in topical cosmetics. Further medical uses require functionalization of C60 to make it soluble and one of the simplest functionalization is to make C60(OH)n fullerenols. A previous article [Adv. Quant. Chem. 8, 351 (2023)] studied reactivity indices for the successive addition of the $^\bullet$OH radical to ($^\bullet$)C$_{60}$(OH)$_n$ in gas phase. [($^\bullet$)C$_{60}$(OH)$_n$ is only a radical when n is an odd number.] This present article extends this previous work by examining various aspects of how the reaction, changes in aqueous solution. One obvious difference between C$_{60}$ and their various isomers of C$_{60}$(OH)$_2$ is the presence of a dipole. As fullerendiols are nearly spherical, their change in dipole moment in going from gas to aqueous phase may be estimated using back-of-the-envellope calculations with the Onsager model. The result is remarkably similar to what is obtained using density-functional theory (DFT) and the more sophisticated solvation model based upon the quantum mechanical density (SMD). Calculation of fullerendiol C-O bond energies and reactivity indices using with the SMD approach confirm that the general conclusions from the earlier work regarding gas-phase reactivity still hold in the aqueous phase.

==> cameroon.tex <==
% ===============================================================
% File cameroon.tex .
% Last modified: 9 July 2024
% ===============================================================

This subsection concerns all 59 isomers and treats the solvent by
using the implicit solvent model.  The first two subsubsections
are concerned, respectively, with chemical properties (reactivity indices)
and with a physical property (dipole moments) which is intimately related
to implicit solvent models.  These calculations were all carried out
without any symmetry breaking---that is using the 
% -------------------------------------
\marginpar{\color{blue} DODS, SODS}
% -------------------------------------
same-orbitals-for-different-spins (SODS) model.  This is followed by
a subsection on PECs for vertical dissociation.  Vertical dissociation
is far from a realistic study of transition states and intrinsic reaction
coordinates but it allows us to get a rapid overview of how the PECs
behave for the dissociation of different isomers into two separate
radicals.  We now introduce symmetry breaking as the minimal acceptable
model for describing the breaking of a bond to form two separate radicals.
As such we are using different-orbitals-for-different-spins (DODs) and
also follow the degree of spin-contamination in the wave function by
looking at how $\langle {\hat S}^2 \rangle$ evolves along each PEC.

% -----------------------------------
\subsubsection{Reactivity Indices}
% -----------------------------------

Reactivity indices calculated within the SMD implicit solvent model are
shown in {\bf Fig.~\ref{fig:SMDReactivityIndices}}.  
These results look very much like the corresponding gas-phase results 
\cite{PEMC23}, which is a nice confirmation that $^\bullet$OH remains
an electrophilic radical in solution even with respect to an ``electron
sponge'' such as C$_{60}$.
% ----------------------
\begin{figure}
\begin{center}
\begin{tabular}{cc}
(a) & \\
% (b) & \includegraphics[width=0.6\textwidth]{./Graphics/2023_03_23_1.eps} \\
(b) & \includegraphics[width=0.6\textwidth]{./Graphics/Fig03a.eps} \\
% (c) & \includegraphics[width=0.6\textwidth]{./Graphics/2023_03_23_2.eps} \\
(c) & \includegraphics[width=0.6\textwidth]{./Graphics/Fig03b.eps} \\
%     & \includegraphics[width=0.6\textwidth]{./Graphics/2023_03_23_3.eps} \\
    & \includegraphics[width=0.6\textwidth]{./Graphics/Fig03c.eps} \\
\end{tabular}
\end{center}
\caption{
B3LYP(VWN3)/def2SVP/SMD reactivity indices calculated with 
an implicit solvent model.
% {\color{red} I do not think that this needs recalculation although
% broken symmetry should change the results a bit.} 
\label{fig:SMDReactivityIndices}
}
\end{figure}
% ---------------------

% -----------------------------------
\subsubsection{Dipole Moments}
% -----------------------------------


% ----------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.8\textwidth]{./Graphics/Onsager2.eps}
\includegraphics[width=0.8\textwidth]{./Graphics/Fig04.eps}
\end{center}
\caption{
Graph correlating the magnitudes of gas-phase and aqueous-phase
dipole moments for C$_{60}$(OH)$_2$ fullerenols calculated using geometries optimized 
in the gas phase. The dashed % red 
line is the result of Onsager's implicit solvent model.  See text.
% {\color{red} I do not think that this needs recalculation although
% broken symmetry should change the results a bit.} 
\label{fig:Onsager}
}
\end{figure}
% ---------------------
The simplest implicit solvent model is the Onsager model which we expect
to be a good first approximation for fullerendiols.  This is confirmed
in {\bf Fig.~\ref{fig:Onsager}} where we a correlation plot between 
calculated gas-phase and aqueous-phase dipole moments.
The Onsager model predicts a straight line 
passing through the origin and with slope,
\begin{equation}
  m = 1 - \left( \frac{2 (\epsilon -1)}{2 \epsilon+1} \right)
  \left( \frac{n^2-1}{n^2+2} \right) \, . 
  \label{eq:SMD.1}
\end{equation}
Here $\epsilon$ is the dielectric constant of the surrounding water,
which is well-known to be close to 80, and $n$ is the refractive index of
solid C$_{60}$ which is 2.2 at 630 nm wavelength \cite{H91}.  Using these 
values gives a slope of $m=0.44906$ which corresponds to the dashed % red 
line in Fig.~\ref{fig:Onsager}.  We can conclude that the Onsager model is a 
reasonable first approximation to the SMD implicit solvent model in this case.

% ----------------------------------------------------------
\subsubsection{Vertical Dissociation PECs}
% ----------------------------------------------------------

PECs have been calculated for reaction~(\ref{eq:results.1})
for rigid vertical removal of $^\bullet$OH without any internal relaxation
of either $^\bullet$C$_{60}$OH or $^\bullet$OH ({\bf Fig.~\ref{fig:vertical}}).
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.7\textwidth]{./Graphics/vertical.eps} 
\includegraphics[width=0.7\textwidth]{./Graphics/Fig05.eps} 
\end{center}
\caption{
Illustration for isomer {\bf 1} of a procedure used for isomers {\bf 1}, 
{\bf 2}, and {\bf 3}.  The vertical docking of $^\bullet$OH on 
$^\bullet$C$_{60}$OH was accomplished by begining from the fullerendiol
and using {\sc Molden} \cite{molden} to construct a Z-matrix.  Then only
the C-O distance was varied for carbon number 1, keeping all other bond
and dihedral angles fixed.  In particular the structures of $^\bullet$OH
and $^\bullet$C$_{60}$OH were kept fixed.
\label{fig:vertical}
}
\end{figure}
% ------------------------------------------------------------------

Symmetry breaking is employed and spin-contamination is followed by
looking at $\langle {\hat S}^2 \rangle$ for all 59 isomers.  Comparisons
are made between gas-phase and solvated PECs for both long and short
distances.  This still means a lot of calculations and time-consuming
analysis, most of which has been relegated to the ESI.  Here we just
focus on a few examples to bring out our principle conclusions.  

To our surprise, it was found that many of the isomers show significant
spin contamination at short (i.e., bonding) distances.  The degree 
of spin contamination for the different isomers is shown in 
{\bf Fig.~\ref{fig:contaminationsites}}.  Values of $\langle {\hat S}^2 \rangle$
vary from 0.00 to about 1.00 (in some cases we see $\langle {\hat S}^2 \rangle$
slightly exceeding 1.00).  This later value is typical of what is expected
for a diradical. 
Interestingly, the sites with zero spin contamination seem almost, but 
not quite, to alternate with sites with significant spin contamination.  
The value of $\langle {\hat S}^2 \rangle = 1$ has already been explained
by the LDS shown in Fig.~\ref{fig:diradical}.  The implications for 
further reactivity with a third $^\bullet$OH radical are evident.
However, we should remember that the unpaired spins may 
be widely distributed around the molecule in a way that corresponds to
multiple diverse resonance structures in the Lewis representation.
The reader is invited to explore which different LDSs may be drawn for
each isomer.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{./Graphics/contaminationsites.eps} 
\end{center}
\caption{
Spin contamination: The numbers show the degree of spin-contamination
at a C-O distance of 1.4 {\AA} for the {\em second} OH group.  Note
that the first OH group is always on carbon 1.  It is important to
note that the underlying figure is the same as in Fig.~\ref{fig:IUPAC}
because many of the carbon numbers are obscured by the red numbers
showing the value of $\langle {\hat S}^2 \rangle$.
\label{fig:contaminationsites}
}
\end{figure}
% ------------------------------------------------------------------

We will just focus on the extreme cases in our discussion, namely
when spin contamination is negligeable along the vertical PEC and
when it is maximal.  The 1,5-C$_{60}$(OH)$_2$ isomer is a case where
spin contamination becomes negligeable below 2.0 {\AA} in the gas-phase
and below 2.2 {\AA} in aqueous solution.  The corresponding PECs and 
values of $\langle {\hat S}^2 \rangle$ along the PEC are shown in 
{\bf Fig.~\ref{fig:PECandS2_5}}.  For reference, the typical
length of a C-O single bond is 1.33-1.43 {\AA} while the van der
Waals radius of water is estimated to be about 2.75-3.2 {\AA} \cite{waterR},
so 1.4-2.0 {\AA} corresponds to a stretched bond within a solvent
excluded volume.  In such a case, we might expect that the PEC in
solution would be parallel to the PEC in gas phase and 
{\bf Fig.~\ref{fig:SRLR_5}}
confirms that the shifted solvent PEC matches the gas-phase PEC
very well at short distance (i.e., below about 1.8 {\AA}).  While it
may appear that there is also a similar matching of curve shape at
long distance, this is really just a consequence of both curves having
to go to zero at dissociation.  We expected the long distance behavior
to go as $1/R^3$ which is typical of a dipole-dipole interaction.  Instead
we were surprised to see a region with a $1/R^6$ van der Waals interaction-like
behavior ({\bf Fig.~\ref{fig:vdW_5}}).  There is a simple argument that 
DFT should be unable to describe the van der Waals $1/R^6$ part of the
potential when the electron density of the separated fragments no longer
overlap.  Our calculations do not contradict this idea as the $1/R^6$
is no longer present at very long distance.  However, this is a reminder
that a good functional can capture some of the $1/R^6$ behavior at 
moderately long distance.  Indeed one of the challenges when adding
van der Waals corrections to DFT is not to overcount any $1/R^6$ behavior
that may be already present in the functional.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{./Graphics/PECandS2_5.eps} 
\end{center}
\caption{
1,5-C$_{60}$(OH)$_2$ (isomer {\bf 6}) vertical dissociation PECs 
and spin-contamination for the same geometries in gas phase and in 
aqueous solution.
\label{fig:PECandS2_5}
}
\end{figure}
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{./Graphics/SRLR_5.eps} 
\end{center}
\caption{
Comparison of the short- and long-range shapes of the solution 
1,5-C$_{60}$(OH)$_2$ (isomer {\bf 6}) vertical dissociation PEC with 
the gas-phase PEC: left, PECs matched at short and long range;
right, corresponding solution-gas phase PEC curves.
\label{fig:SRLR_5}
}
\end{figure}
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{./Graphics/vdW_5.eps} 
\end{center}
\caption{
Identification of the van der Waals region of the 1,5-C$_{60}$(OH)$_2$ 
(isomer {\bf 6}) vertical dissociation PECs. The upper row shows log-log 
plots of the PEC and tries to ``fit'' the van der Waals region. The lower 
row uses a finite difference method to calculate the derivative and then 
does a least-squares fit to a cubic polynomial.
\label{fig:vdW_5}
}
\end{figure}
% ------------------------------------------------------------------

Now let us look at a case with where spin contamination is high at 1.4 {\AA}.
We choose to look at 1,6-C$_{60}$(OH)$_2$ which has a spin contimanation of
about $\langle {\hat S}^2 \rangle = 1.00$ at 1.4 {\AA}.  The PECs and 
values of $\langle {\hat S}^2 \rangle$ along the PEC are shown in 
{\bf Fig.~\ref{fig:PECandS2_7}}.  Judging from $\langle {\hat S}^2 \rangle$,
one might suppose that the two approaching radicals remain radicals without
forming a bond.  However the PECs indicate clear bonding, meaning that
the unpaired electrons have moved onto the C$_{60}$ moiety.  Perhaps
unexpectedly, the short-range behavior in solution no longer parallels
the short-range behavior in gas phase ({\bf Fig.~\ref{fig:SRLR_7}}).
In fact, this only seems to occur in cases where there is no spin contamination
at short distance.  On the other hand, {\bf Fig.~\ref{fig:vdW_7}}
shows a significantly enlarged $1/R^6$ region.  This is also typical
of what is seen in other isomers with significant spin contamination.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{./Graphics/PECandS2_7.eps} 
\end{center}
\caption{
1,6-C$_{60}$(OH)$_2$ (isomer {\bf 7}) vertical dissociation PECs 
and spin-contamination for the same geometries in gas phase and in 
aqueous solution.
\label{fig:PECandS2_7}
}
\end{figure}
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{./Graphics/SRLR_7.eps} 
\end{center}
\caption{
Comparison of the short- and long-range shapes of the solution 
1,6-C$_{60}$(OH)$_2$ (isomer {\bf 7}) vertical dissociation PEC with 
the gas-phase PEC: left, PECs matched at short and long range;
right, corresponding solution-gas phase PEC curves.
\label{fig:SRLR_7}
}
\end{figure}
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\includegraphics[width=0.9\textwidth]{./Graphics/vdW_7.eps} 
\end{center}
\caption{
Identification of the van der Waals region of the 1,6-C$_{60}$(OH)$_2$ 
(isomer {\bf 7}) vertical dissociation PECs. The upper row shows log-log 
plots of the PEC and tries to ``fit'' the van der Waals region. The lower 
row uses a finite difference method to calculate the derivative and then 
does a least-squares fit to a cubic polynomial.
\label{fig:vdW_7}
}
\end{figure}
% ------------------------------------------------------------------

%%%%%%%
% EOF %
%%%%%%%


==> compare.tex <==
% ===============================================================
% File compare.tex .
% Last modified: 15 June 2024
% ===============================================================

As {\sc LICHEM} calculations are much more computer resource intensive
than SMD implicit solvent calculations, we have found that the best
way to obtain some information about the {\sc LICHEM} calculations is
by comparing against more easily analyzed implicit solvent calculations
using the same geometries generated using {\sc LICHEM}.

% ---------------------------------------------------------
\begin{table}
\begin{tabular}{ccccc}
\hline \hline
$^\bullet$OH & Isomer & $^\bullet$C$_{60}$OH & Total & Relative \\
\hline
\multicolumn{5}{c}{Gas Phase} \\
-75.667309457297 Ha & {\bf 1} & -2360.260006969341 Ha & 
-2435.927316426638 Ha & -3.77 kcal/mol \\
-75.667360194518 Ha & {\bf 2} & -2360.253951146379 Ha &    
-2435.9213113408973 Ha & 0.00 kcal/mol \\  % highest energy
-75.667350287007 Ha & {\bf 3} & -2360.260537252224 Ha &  
-2435.927887539231 Ha & -4.13 kcal/mol \\  
\multicolumn{5}{c}{Aqueous Solution} \\
-75.675569232329 Ha & {\bf 1} & -2360.283439313127 Ha & 
-2435.959008545456 Ha & -3.66 kcal/mol \\
-75.675570505525 Ha & {\bf 2} & -2360.277602169459 Ha &   
-2435.9531726749838 Ha & 0.00 kcal/mol \\  % highest energy
-75.675621197244 Ha & {\bf 3} & -2360.284318607294 Ha & 
-2435.959939804538 Ha & -4.25 kcal/mol \\
\hline \hline
\end{tabular}
\caption{
\label{tab:productenergies}
Product energies for the three isomers {\bf 1}, {\bf 2}, and {\bf 3}
calculated using {\sc Gaussian} at the B3LYP(VWN3)/def2SVP in gas
phase and using the SMD implicit solvation model for aqeous solvation
using the same products used in our {\sc LICHEM} calculations.
}
\end{table}
% ---------------------------------------------------------
For example, one thing that is more easily calculated using the SMD
method is the energy of the infinitely separated products.  This is shown
in {\bf Table~\ref{tab:productenergies}} where we also see that 
conformational energy differences between the product $^\bullet$C$_{60}$OH
is as large as 4.25 kcal/mol, which is small but still non-negligeable compared
with the binding energies of the reactants.  This allows us to put our
relative energy PECs on a common absolute scale in {\bf Fig.~\ref{fig:waterIRC}}.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\begin{tabular}{cc}
(a) &  \\
% (b) & \includegraphics[width=0.6\textwidth]{./Graphics/waterIRCdef2SVP2.eps} \\
(b) & \includegraphics[width=0.6\textwidth]{./Graphics/Fig10a.eps} \\
%    & \includegraphics[width=0.6\textwidth]{./Graphics/waterS2def2SVP.eps} 
    & \includegraphics[width=0.6\textwidth]{./Graphics/Fig10b.eps} 
\end{tabular}
\end{center}
\caption{
Aqueous-phase B3LYP(VWN3)/def2SVP//SMD PECs calculated 
with {\sc Orca} along the {\sc LICHEM} aqueous-phase IRCs calculated at the
B3LYP(VWN)/6-31G//AMBER level: (a) PECs, {\color{red} shifted relative to the
sum of the energies of the individual product radicals in solution}. (b) The
corresponding values of $\langle \hat{S}^2 \rangle$. 
\label{fig:waterIRC}
}
\end{figure}
% ------------------------------------------------------------------

We may now compare our implicit solvent ({\sc Orca} SMD) with the
our explicit solvent ({\sc LICHEM}) PECs.  If the agreement is acceptable,
then we may continue our analysis with the implicit solvent calculations.
The PEC comparison is shown in {\bf Fig.~\ref{fig:JandA_PECs}}.
Only semi-quantitative agreement is expected and indeed this is what we
find.  But it is good enough to authorize further analysis with the implicit
solvent model.
% ----------------------
\begin{figure}
\begin{center}
\begin{tabular}{c}
(a) 1,9-C$_{60}$(OH)$_2$ ({\bf 1}) \\
% \includegraphics[width=0.5\textwidth]{./Graphics/JorgeAndAbrahamPECinWater1.eps} \\
\includegraphics[width=0.5\textwidth]{./Graphics/Fig11a.eps} \\
(b) 1,8-C$_{60}$(OH)$_2$ ({\bf 2}) \\
% \includegraphics[width=0.5\textwidth]{./Graphics/JorgeAndAbrahamPECinWater2.eps} \\
\includegraphics[width=0.5\textwidth]{./Graphics/Fig11b.eps} \\
(c) 1,7-C$_{60}$(OH)$_2$ ({\bf 3}) \\
% \includegraphics[width=0.5\textwidth]{./Graphics/JorgeAndAbrahamPECinWater3.eps} \\
\includegraphics[width=0.5\textwidth]{./Graphics/Fig11c.eps} \\
\end{tabular}
\end{center}
\caption{
{\sc LICHEM} explicit solvent B3LYP(VWN3)/6-31G//AMBER and 
{\sc Orca} implicit solvent B3LYP(VWN3)/6-31G//SMD results
in aqueous solution.
{\color{red} Notes: This could be in black and white.  The reactant-to-product
values of the C-O bond distance have been ``sort of guessed'' because Jorge
did not supply them.  These calculations are broken symmetry singlet 
calculations.  They should be redone using the def2SVP basis set.  We
should also analyze the short and long range behavior of these curves.
The short-range behavior involves comparsing with the gas-phase PECs.
The long-range behavior involves knowing the angle between the two OHs.}
\label{fig:JandA_PECs}
}
\end{figure}
% --------------------

In particular, we are able to say something about symmetry breaking.
Equation~(\ref{eq:results.1}) describes the breaking of single bond to form
two radicals.  This is a famous strongly-correlated problem because
single-determinantal wave functions lead to dissociation at too high an
energy.  The usual way around this in DFT is to simulate the effects of
a multideterminantal calculation by allowing the orbitals to break spatial
symmetry so that we have different orbitals for different spin.  At the
Coulson-Fischer point, the spin-broken solution will become lower than 
the spin-restricted (same orbitals for different spin) energy.  One way to
find the Coulson-Fischer point is to monitor the value of 
$\langle \hat{S}^2 \rangle$ in the symmetry-broken calculation.  The
theoretical pure spin-state eigenvalue of $\langle \hat{S}^2 \rangle$
is $S(S+1)$ which is 0 for a singlet and 2 for a triplet.  At the 
Coulson-Fischer point, $\langle \hat{S}^2 \rangle$ will depart from zero
towards a larger value and become unity for a diradical.  (See, e.g., 
Ref.~\cite{MC17}.)

The aqueous-phase values of $\langle \hat{S}^2 \rangle$
calculated by {\sc Orca} along the {\sc LICHEM} QSM aqueous-phase IRCs
are shown in Fig.~\ref{fig:waterIRC}(b).
% Energies are relative to the dissociation products $^\bullet$OH and
% $^\bullet$C$_{60}$OH shown in {\bf Table~\ref{tab:productenergies}}.
% Note that there are three different energies for $^\bullet$C$_{60}$OH
% because, although dissociation of the isomers leads to a single
% isomer, each isomer has several possible conformations.
For isomers {\bf 1} and {\bf 3},
the Coulson-Fischer point is at around 2 {\AA}.  At larger distances,
the value of $\langle \hat{S}^2 \rangle$ increases and approaches unity
at complete dissociation.  This is entirely expected and reassures us that
the C-O bond is dissociating correctly.  However, the 
$\langle \hat{S}^2 \rangle$ curve for isomer {\bf 2} is different since
it descends as the C-O bond distances decreases and then suddenly increases
at smaller C-O distances towards the value corresponding to a diradical.
This confirms the diradical representation that we have shown in 
Fig.~\ref{fig:diradical}.  It also explains the markedly higher energy
of isomer {\bf 2} than either of isomers {\bf 1} or {\bf 3} at bonding
distances.  We have also carried out the gas-phase calculations along the same
pathway and these are shown in {\bf Fig.~\ref{fig:gasIRC}} which shows the
same general phenomenon.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\begin{tabular}{cc}
(a) &  \\
% (b) & \includegraphics[width=0.6\textwidth]{./Graphics/gasIRCdef2SVP2.eps} \\
(b) & \includegraphics[width=0.6\textwidth]{./Graphics/Fig12a.eps} \\
%    & \includegraphics[width=0.6\textwidth]{./Graphics/gasS2def2SVP.eps} 
    & \includegraphics[width=0.6\textwidth]{./Graphics/Fig12b.eps} 
\end{tabular}
\end{center}
\caption{
Gas-phase B3LYP(VWN3)/def2SVP PECs calculated with {\sc Orca} 
along the {\sc LICHEM} aqueous-phase IRCs calculated at the
B3LYP(VWN)/6-31G//AMBER level: (a) PECs, {\color{red} shifted relative to the
sum of the energies of the isolated product radicals}. (b) The
corresponding values of $\langle \hat{S}^2 \rangle$. 
\label{fig:gasIRC}
}
\end{figure}
% ------------------------------------------------------------------

{\color{red}
The question then arises as to where the unpaired spins are located in 
isomer {\bf 2}.  {\bf Figure~\ref{fig:gasspinddensity}} shows the 
Mulliken population spin-density for isomer {\bf 2}.  
Consistent with the expectations of Fig.~\ref{fig:diradical},
the highest spin densities (of opposing sign) are at carbons 7 (spin up)
and 9 (spin down).  
The interested reader is invited to draw resonance structures and to
try to assign relative weights consisted with all of these calculated
spin densities.}  {\color{magenta} This shows that the neglect of symmetry
breaking in our exploratory calculations was na\"{\i}ve, though still 
useful as an initial exploratory calculation.}
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.8\textwidth]{./Graphics/gasspindensity.eps}
\includegraphics[width=0.8\textwidth]{./Graphics/Fig13.eps}
\end{center}
\caption{
Gas-phase Mulliken population spin-density 
calculated with {\sc Orca} for 1,8-C$_{60}$(OH)$_2$ (isomer {\bf 2}) 
[calculated at the B3LYP(VWN3)/def2SVP level and a C$_1$-O distance 
of 1.47 {\AA}]. (IUPAC numbering shown in Fig.~\ref{fig:IUPAC}.)
\label{fig:gasspinddensity}
}
\end{figure}
% ------------------------------------------------------------------

\begin{verbatim}

  +------+
  | STOP |
  +------+

\end{verbatim}


{\color{red} I also want to analyze the long- and short-range behavior of the 
PECs, but I think that this will be best done for the vertical dissociation
in {\tt cameroon.tex}. Nevertheless, I am leaving this for now:}


{\bf Figure~\ref{fig:dipoledipole}} compares the behavior of a log-log 
(or, more exactly, ln-ln) plot of the three PECs with the expected
line of slope $m=-3$ for an energy dominated by the interaction of
the two OH bond dipole moments.  From 
% Eq.~(\ref{eq:vdW.2}), we expect,
the potential between two fixed point dipole moments is
\begin{equation}
  U_{d-d}^{\mbox{fixed}} = \frac{{\vec \mu}_1 \cdot {\vec \mu}_2 -
  3 ({\vec \mu}_1 \cdot \hat{R}) ({\vec \mu}_2 \cdot \hat{R})}{\epsilon R^3} 
  \, ,
  \label{eq:vdW.2}
\end{equation}
we expect,
\begin{equation}
  \mbox{ln} U_{d-d}^{\mbox{fixed}} = -3 \mbox{ln} R + \mbox{ln} \left[
  {\vec \mu}_1 \cdot {\vec \mu}_2 - 3({\vec \mu}_1 \cdot {\hat R})
  ({\vec \mu}_2 \cdot {\hat R}) \right]
  -\mbox{ln} \epsilon \, ,
  \label{eq:line}
\end{equation}
where $\mbox{ln} \epsilon = 0$ in the gas phase.  The intercept of the 
line depends upon the orientation between the two OH bond dipole moments 
which differs for the three IRCs.  Consider vertical removal of an OH group
and Fig.~\ref{fig:diradical}.  The term 
$({\vec \mu}_1 \cdot {\hat R}) ({\vec \mu}_2 \cdot {\hat R})$
is expected to be roughly independent of the isomer, so we may focus
on the ${\vec \mu}_1 \cdot {\vec \mu}_2$ term whose magnitude we expect
to be roughly in the order: {\bf 1} $\approx$ {\bf 2} $>$ {\bf 3}.
Thus the theoretical dipole-dipole line for isomer {\bf 3} should fall 
below the theoretical dipole-dipole lines for isomers {\bf 1} and {\bf 2}.
This appears to be what we are seeing in Fig.~\ref{fig:dipoledipole}.
Note, however, that the angle between the two OH bonds varies along each 
IRC as the OH groups try to maintain hydrogen bonds during the dissociation
(see the films in the ESI).
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.8\textwidth]{./Graphics/gasdipoledipole2.eps} 
\includegraphics[width=0.8\textwidth]{./Graphics/Fig14.eps} 
\end{center}
\caption{
Log-log plot of the gas-phase B3LYP(VWN3)/def2SVP PECs calculated with 
{\sc Orca} along the {\sc LICHEM} aqueous-phase IRCs calculated at the
B3LYP(VWN)/6-31G//AMBER level.  The dashed lines are the expected 
lines with $m=-3$ slope for asymptotic energies dominated by interactions
between the two OH bond dipole moments.
\label{fig:dipoledipole}
}
\end{figure}
% ------------------------------------------------------------------

{\bf Figures~\ref{fig:waterIRC}} and {\bf \ref{fig:waterdipoledipole}}
show that the same analysis also applies in aqueous solution.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.8\textwidth]{./Graphics/waterdipoledipole2.eps} 
\includegraphics[width=0.8\textwidth]{./Graphics/Fig15.eps} 
\end{center}
\caption{
Log-log plot of the aqueous-phase B3LYP(VWN3)/def2SVP//SMD PECs calculated with 
{\sc Orca} along the {\sc LICHEM} aqueous-phase IRCs calculated at the
B3LYP(VWN)/6-31G//AMBER level.  The dashed lines are the expected 
lines with $m=-3$ slope for asymptotic energies dominated by interactions
between the two OH bond dipole moments.
\label{fig:waterdipoledipole}
}
\end{figure}
% ------------------------------------------------------------------



%%%%%%%
% EOF %
%%%%%%%


==> texas.tex <==
% ===============================================================
% File texas.tex .
% Last modified: 15 June 2024
% ===============================================================

% ---------------------------------------
\subsubsection{Potential Energy Curves}
% ---------------------------------------

% ------------------------------------------------------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.6\textwidth]{./Graphics/vmdscene.eps}
\includegraphics[width=0.6\textwidth]{./Graphics/Fig06.eps}
\end{center}
\caption{
Isomer {\bf 1} in a box of water in our QM/MM treatment.  1,9-C$_{60}$(OH)$_2$
is treated at the QM level while the water molecules are treated at the 
MM level.
\label{fig:vmdscene}
}
\end{figure}
% ------------------------------------------------------------------
{\color{blue} Broken symmetry (DODS) {\sc LICHEM} calculations of PECs 
were carried out for the three isomers shown in Fig.~\ref{fig:diradical}.  
These are QM/MM calculations ({\bf Fig.~\ref{fig:vmdscene}}) for which we
carry out QSM calculations which resemble nudged elastic band calculations
in that reactant and product geometries are specified and the lowest
energy path is sought between them.  This was done in aqueous solution
% -------------------------------------
\marginpar{\color{blue} R2P}
% -------------------------------------
going both in the reactants-to-products (R2P) direction and then back in the
products-to-reactants (P2R) direction.  This gives a set of geometries close
% -------------------------------------
\marginpar{\color{blue} IRC}
% -------------------------------------
to the intrinsic reaction coordinate (IRC) in solution, but which 
contain statistical variations due primarily to the exact procedure
followed in our calculations---namely that the solvent environment at
the starting point (i.e., reactant or product) is obtained via a separate
finite temperature MD calculation.  During the QSM calculation, solvent
molecules within a certain distance of the reaction center are allowed to
readjust to minimize the free energy along the QSM.  As the starting 
solvent configurations for the QSM are different for the product-to-reactant
and reactant-to-product calculations, it follows that we expect to see
some differences in the calculated IRCs.  This may be taken as an indication
of the statistical error inherent in this particular variant of an MD calculation.  

Results of this procedure, including the expected statistical error, are shown 
in {\bf Fig.~\ref{fig:QSMlichemPEC}}.  The R2P and P2R results are very close at each end
of their respective quadratic strings, but differ somewhat in between for the reasons 
already explained.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\begin{tabular}{cc}
(a) &  \\
% (b) & \includegraphics[width=0.6\textwidth]{./Graphics/QSMlichemPECa3.eps} \\
(b) & \includegraphics[width=0.6\textwidth]{./Graphics/Fig07a.eps} \\
%    & \includegraphics[width=0.6\textwidth]{./Graphics/QSMlichemPECb3.eps}
    & \includegraphics[width=0.6\textwidth]{./Graphics/Fig07b.eps}
\end{tabular}
\end{center}
\caption{
{\color{red} B3LYP(VWN3)/def2-SVP//Amber} QSM PECs calculated with 
{\sc LICHEM} in the aqueous phase: (a) Energy relative to dissociation.  
(b) Log-log plot.  The black line has a slope of -3, typical of the 
potential energy between two dipole moments.
\label{fig:QSMlichemPEC}
}
\end{figure}
% ------------------------------------------------------------------

As {\sc LICHEM} has no good way to calculate the energies of the separated
products, except to use computationally very heavy statistical averaging (not
done here), our primary indication of the correct dissociation into two radicals
is given by the convergence of the singlet and triplet states to the same energy 
({\bf Fig.~\ref{fig:JorgePECinWater}}).
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
\begin{tabular}{cc}
% \includegraphics[width=0.45\textwidth]{./Graphics/COIsomer1R2P.eps} &
\includegraphics[width=0.45\textwidth]{./Graphics/Fig08aa.eps} &
% \includegraphics[width=0.45\textwidth]{./Graphics/COIsomer1P2R.eps} \\
\includegraphics[width=0.45\textwidth]{./Graphics/Fig08ab.eps} \\
% \includegraphics[width=0.45\textwidth]{./Graphics/COIsomer2R2P.eps} &
\includegraphics[width=0.45\textwidth]{./Graphics/Fig08ba.eps} &
% \includegraphics[width=0.45\textwidth]{./Graphics/COIsomer2P2R.eps} \\
\includegraphics[width=0.45\textwidth]{./Graphics/Fig08bb.eps} \\
% \includegraphics[width=0.45\textwidth]{./Graphics/COIsomer3R2P.eps} &
\includegraphics[width=0.45\textwidth]{./Graphics/Fig08ca.eps} &
% \includegraphics[width=0.45\textwidth]{./Graphics/COIsomer3P2R.eps}
\includegraphics[width=0.45\textwidth]{./Graphics/Fig08cb.eps}
\end{tabular}
\end{center}
\caption{
{\bf LICHEM} PECs for the three isomers in aqueous solution 
(QM/MM) ({\color{red} B3LYP(VWN3)/def2SVP//AMBER}) along the QSM 
optimization path.  Note that the triplet and 
singlet states go to the same energies at large distance which is 
expected for dissociation into two radicals.
\label{fig:JorgePECinWater}
}
\end{figure}
% ------------------------------------------------------------------
} % end blue


% \begin{verbatim}
% 
%   +------+
%   | STOP |
%   +------+
% 
% \end{verbatim}

% ---------------------------------------
\subsubsection{Noncovalent Interactions}
% ---------------------------------------
Weitao Yang and co-workers introduced the reduced density gradient,
\begin{equation}
  s({\vec r}) = \frac{1}{2(3\pi^2)^{1/3}} \frac{\vert {\vec \nabla} 
              \rho({\vec r}) \vert }{\rho^{4/3}({\vec r})} \, ,
  \label{eq:NCI}
\end{equation}
% -------------------------------------
\marginpar{\color{blue} NCI}
% -------------------------------------
as an indicator of noncovalent interactions (NCIs) 
\cite{JKMC+10,CYJ11,PC17}.  {\bf Figure~\ref{fig:NCI}} shows snapshots from a film
of the NCI along the reaction path.  These snapshots contain a lot of information.
For example, dotted lines show hydrogen bonds that are breaking and reforming between
water molecules in the MM part of the simulation and between MM and QM water molecules.
Close examination of the water molecules, particularly in the intermediate times show
that this is actually a superposition of the R2P and P2R simulations, which are nearly
identical.  Also shown is the NCI.  Strong NCIs are shown in red and appear in the center
of the faces of the fullerene part of the system and also as the C-O bond forms.  Green
NCIs signal the presence of hydrogen bonding.  For isomer {\bf 1}, this is evident in
the far left when the fullerendiol is dissociated but hydrogen bonding still occurs between
$^\bullet$OH and $^\bullet$C$_{60}$OH.  For isomer {\bf 2}, hydrogen bonding appears to 
occur between the C and O as the two begin to react.  It is not clear that this should
be called a hydrogen bond.  However the middle figure shows a clear H-O$\cdots$H-O hydrogen
bond.  No true hydrogen bonding is noticable along the pathway for isomer {\bf 3}.
% ------------------------------------------------------------------
\begin{figure}
\begin{center}
% \includegraphics[width=0.8\textwidth]{./Graphics/NCI.eps}
\includegraphics[width=0.8\textwidth]{./Graphics/Fig09.eps}
\end{center}
\caption{
NCI snapshots of a film for the reaction of $^\bullet$OH with $^\bullet$C$_{60}$OH
to form isomers {\bf 1}, {\bf 2}, and {\bf 3}.
\label{fig:NCI}
}
\end{figure}
% ------------------------------------------------------------------


{\color{red}
\begin{verbatim}

I agree with most of the points by Mark above except for the last point, point 4). 
The reason is that when the PESs (I prefer the term surfaces to curves personally) 
for the QSM calculated MEPs starting with the initial guess using either one or the 
other minima ("forward" or "backward" in the previous terminology) it is clear that 
the energy changes for intermediate images, this was the plot that Mark prepared for 
our last meeting.  In the figures that Jorge sent it is also observed that there are 
slight, but visible differences on the arrangement of the environmental waters, which 
shows that the differences in energy for these points is directly related to the 
explicit solvation environment. And since we don't have any sampling we can't say that 
it is averaged out.  As for the intra-molecular H-bond, i.e. bonding to the OH already 
bound to C60, there is also noticeable changes on how this affects the energies as 
shown by the NCI index surfaces.

\end{verbatim}
How can we work in Andr\'es comments?  Also, I think we should refer here to 
Refs.~\cite{WCL+14,KT17,WGZ18}.
}


%%%%%%%
% EOF %
%%%%%%%

